Robust Nonparametric Regression under Huber's $\epsilon$-contamination Model

We consider the non-parametric regression problem under Huber's $\epsilon$-contamination model, in which an $\epsilon$ fraction of observations are subject to arbitrary adversarial noise. We first show that a simple local binning median step can effectively remove the adversary noise and this median estimator is minimax optimal up to absolute constants over the H\"{o}lder function class with smoothness parameters smaller than or equal to 1. Furthermore, when the underlying function has higher smoothness, we show that using local binning median as pre-preprocessing step to remove the adversarial noise, then we can apply any non-parametric estimator on top of the medians. In particular we show local median binning followed by kernel smoothing and local polynomial regression achieve minimaxity over H\"{o}lder and Sobolev classes with arbitrary smoothness parameters. Our main proof technique is a decoupled analysis of adversary noise and stochastic noise, which can be potentially applied to other robust estimation problems. We also provide numerical results to verify the effectiveness of our proposed methods.

==> conclusion.tex <==
In this paper we proposes and analyzed the first computationally efficient method for robust nonparametric regression problem in Huber's $\epsilon$-contamination model.
Our method uses median operation and standard kernel smoothing and achieves minimax optimal contamination dependency and statistical rate for \holder function class.
Further, our estimator does not require known contamination parameter $\epsilon$.
In the following we list some future directions.

%adaptiveity
Though our estimator does not require known contamination parameter $\epsilon$, we do need to know the smoothness $(\beta)$ and Lipschitz constant $(L)$ for \holder class.
A natural question is how to design estimators when these parameters are unknown.
There has been extensive works in statistic literature on this adaptivity problem, e.g. Lepski method`~\citep{lepskii1991problem} and wavelet block-thresholding~\citep{cai1999adaptive}.
We may try to adapt these procedures in Huber's $\epsilon$-contamination model.


%other function class
Another interesting direction in to consider estimating functions in other classes rather than \holder, like Sobolev and Besov spaces.
We believe if the function class can be embedded in a \holder class, then our local binning median procedure can still be used as a preprocessing step.

%strong adversarial model
Lastly, in this paper, we only consider uniform adversarial model, i.e., each observation has $\epsilon$ probability subject to an adversarial noise.
A stronger adversarial model is the adversary can choose $\epsilon n$ points to inject noise.
Note in this setting, our local binning median estimator does not work because adversary can more than $s/2$ points in a local region and completely ruin the estimation locally.
What is the minimax rate and how to design efficient method for this strong adversarial model is an open problem.


==> main.tex <==
\subsection{Fixed Design with Huber's Contamination Model}





\subsection{Fixed Design with Fully Adversary Noise~\cite{diakonikolas2016robust}}
In this model, there is no hope to obtain an $L_\infty$ norm bound but only $L_2$.
Let $L$ be the upper bound of $f$, if it is not known we can use the median of all data to have a rough estimate.
We have $\epsilon n$ adversarial points and $T$ bins.
Suppose there are $n_1,\cdots,n_T$ adversarial points in each bin whose sum is equals to $\epsilon n$.
Note $\epsilon_i \le m/2$ because adding more adversarial points will not help for destroying our median estimator.
We will need a new median lemma for fully adversary noise.


\subsection{Random Design with Huber's Contamination Model}
Consider the model\begin{align*}
P_f: X\sim \unif\left[0,1\right], Y \sim N\left(f\left(X\right),1\right).
\end{align*}
For each bin, it is easy to see up to log factor, there are $n/T$ good points, which is similar to the above case.




\subsection{Auxiliary Lemmas for Median}







\begin{lem}\label{thm:adversary_median_m_choose_k}
	Among $x_1,\cdots,x_m$, there are $k$ comes from $Q$ and $\left(n-k\right)$ comes from $P$ where $Q$ is an arbitrary adversarial distribution and $P$ is a known distribution.
	For $m,k$ large enough, let $t^*$ be $\prob\left(y \ge t^*\right) \le  \frac{m/2-k}{m-k} -\frac{\sqrt{2\log\left(1/\delta\right)}}{m-k}$ for $y \sim P$, then \begin{align*}
	\prob\left(\median \left\{x_i\right\}_{i=1}^m > t^*\right) \le \delta.
	\end{align*}
\end{lem}
\begin{proof}
Without loss of generality, let $x_1,\cdots,x_k$ be instances coming from $Q$ and $x_{k+1},\cdots,x_m$ be instances coming from $P$.
If $\median\left\{x_i\right\}_{i=1}^m$ is bigger than $t$ then at least $m/2 - k$ instances from $x_{k+1},\cdots,x_m$ are bigger than $t$.
Let $p_t$ be the probability $y \ge t$ where $t \sim P$ and $S_m =\sum_{i=k+1}^{m}\indicator\left[x_i \ge t^*\right]$.
Therefore, \begin{align*}
& \prob\left(\median \left\{x_i\right\}_{i=1}^m > t^*\right)  \\
\le  & \prob\left(S_m \ge \frac{m}{2}-k\right) \\
= & \prob\left(S_m \ge \left(m-k\right)p_t + \left(m/2-k-\left(m-k\right)p_t\right)\right) \\
\le & \exp\left(\frac{-\left(\frac{\left(m/2-k-\left(m-k\right)p_t\right)}{\left(m-k\right)p_t}\right)^2\left(m-k\right)p_t}{2}\right) \\
\le & \delta.
\end{align*}
The first inequality because the worst case is that all $\left\{x_i\right\}_{i=1}^k$ are larger than $t^*$
The second inequality is by Chernoff bound on binomial distribution.
The third inequality is by our choice of $p_t$.
\end{proof}







Assume we know an upper bound of $f$: $L$.
If in a bin the estimated $\hat{f}$ is larger than $L$ we simply replace it by $L$.
There are totally $\epsilon n$ adversarial points.
Let $n_1,\cdots,n_T$ be number of adversarial points in each bin.
For Gaussian noise, according to Lemma~\ref{thm:adversary_median_m_choose_k}, our loss is with probability $1-\delta$, \begin{align*}
	R = \sum_{i=1}^{T} \left(\min\left\{\frac{n_i}{2\left(m-n_i\right)}+\sqrt{\frac{2\log\left(1/\delta\right)}{m-n_i}},L\right\} \right) /T+ \lambda\left(\frac{m}{n}\right)^{\alpha}.
\end{align*}
Note since $\sum_{i=1}^{n}n_i = \epsilon n$, treating $L$ as a constant there are at most $O\left(\epsilon n/M \right)$ bins have error $L$.
Therefore \[
R \le O\left(\epsilon + \lambda\left(\frac{m}{n}\right)^\alpha +  
\sum_{i=1}^{T} \left(\frac{n_i}{2\left(m-n_i\right)}+\sqrt{\frac{2\log\left(1/\delta\right)}{m-n_i}} \right) /T\right)
\] subject to $n_i \le m/2$.
Therefore we can further bounded it by\begin{align*}
	R \le &O\left(\epsilon + \lambda\left(\frac{m}{n}\right)^\alpha +  2\sqrt{\log\left(1/\delta\right)/m} + 
	\sum_{i=1}^{T} \frac{n_i}{Tm}\right) \\
	= & O\left(\epsilon + \lambda\left(\frac{m}{n}\right)^\alpha +  2\sqrt{\log\left(1/\delta\right)/m} + 
	\frac{\epsilon n}{n}\right) \\
	= & O\left(\epsilon + \lambda\left(\frac{m}{n}\right)^\alpha +  2\sqrt{\log\left(1/\delta\right)/m}\right)
\end{align*}
which has the same rate as before.


==> pre.tex <==
We consider one dimensional fixed design nonparametric regression problem in the Huber's $\epsilon$-contamination model.
Specifically, we let $x_i = \frac{i}{n}$ for $i=0,\ldots,n$ be the design points and we observe $y_i \sim f\left(x_i\right) + \xi_i$ where \[
\xi_i \sim (1-\epsilon )P+ \epsilon Q
\]where $P = N(0,1)$ is the Gaussian distribution with $0$ mean and variance $1$ and $Q$ is an arbitrary adversarial noise.
\footnote{
	We assume Gaussian noise for simplicity of presentation and analysis. 
	It is straightforward to generalize our result to sub-Gaussian random noise.}
In this model, the distribution $Q$ is allowed to be completely arbitrary and represents the distribution of “outliers”. As no restriction is placed on $Q$ the sampled outliers can be gross outliers, i.e. starkly distinct
from $P$ or more subtle outliers which are more difficult to tease apart from
samples. 
An alternative viewpoint arises from the observations that the set of
possible distributions $x_i$ is equivalent to the $\ell_1$ ball around $P$ of radius $\epsilon$. 
Indeed, we can alternatively view desirable estimators in this model as those that are robust to model-misspecification (in the $\ell_1$ or total variation
metric). 

Throughout this paper, we focus on estimating a function $f$ belong to the \holder class.
\begin{defn} \holder function class with smoothness $\beta$ and Lipschitz constant $L$ is defined as
\begin{align*}\Lambda\left(\beta, L\right) = \{
f: \abs{f^{(\ell)}\left(x\right) - f^{(\ell)}\left(y\right)} \le L \abs{x-y}^{\beta - \ell} \\
\abs{f^{(k)}} \le L \text{ for }k=1,\ldots,\ell
\}
\end{align*}where $\ell = \lfloor \beta \rfloor$.
\end{defn}
Intuitively, if a function belongs to this class, its function value and derivatives can only change smoothly.
Many real world regression function is believed to belong to this class~\citep{wasserman2006all,gyorfi2006distribution}.

%We use the square $\ell_2$ as the error metric:\[
%\norm{\hat{f}-f}_2^2 = \left(\int_{0}^{1}\abs{\hat{f}(x)-f(x)}^2 dx\right).
%\]

%Kernel smoothing
It is well-known that if $\xi$ has Gaussian distribution, the classical kernel smoothing estimator~\citep{friedman2001elements,gyorfi2006distribution} achieves the optimal statistical rate.
To construct a kernel smoothing estimator, we consider a kernel function $K(\cdot)$ satisfying the following properties.
\begin{align*}
K(x) \text{ is supported on } [0,1], &\int_{0}^{1}K(x)dx = 1,\\ 
\int_{0}^{1} K(x) x^k dx &= 0 \text{ for } k=1,\ldots,\ell, \\
\int_{0}^{1} K^2(x) dx &= \kappa < \infty.
\end{align*}
Given $0 < h < 1/2$ and a query point $x \in \left(h,1-h\right)$ we define for $i=0,\ldots, n-1$,\begin{align}
K_i^h(x) = \int_{x_j}^{x_{j+1}}\frac{1}{h}K\left(\frac{x-u}{h}\right) du. \label{eqn:kernel_def}
\end{align}
%\simon{Haven't considered boundary effect for kernell smoothing yet. May need to use kernels in~\citep{wang2008effect}.}

Here the bandwidth parameter $h > 0$ is used to control the size of the “neighborhood” of a certain test point $x_0 \in \left[0,1\right]$ in which training points are considered and smoothed. 
A small bandwidth $h$ will have fewer effective training points rendering the variance of the resulting estimate large, while a large bandwidth h tends to “over-smooth” the unknown function over a large domain.


Given these definitions, the kernel smoothing estimator is just the weighted sum of the observations \begin{align*}
\hat{f}(x) = \sum_{i=1}^{n}\frac{1}{h}K_{i}^h(x)y_i.
\end{align*}

For Gaussian noise, kernel smoothing achieves the optimal statistical rate $\asymp n^{-\frac{2\beta}{2\beta+1}}$.
In our setting, the noise is a mixture of Gaussian and an adversarial distribution.
Using the technique developed by~\cite{chen2015robust}, we can derive a minimax lower bound.
\begin{thm}[Minimax Lower Bound for \holder Function Class in Huber's $\epsilon$-contamination Model]
	\label{thm:lower_bound_for_holder}
	\begin{align*}
	\inf_{\hat{f}}\sup_{f \in \Lambda\left(\beta,L\right)}\sup_Q\prob_{\epsilon,f,Q}\left\{\norm{\hat{f}-f}_2^2 \ge 
	\right.\\ \left. C\left(\poly\left(L\right)n^{-\frac{2\beta}{2\beta+1}}+\epsilon^2\right)\right\} \ge c
	\end{align*} for some absolute positive constants $C$ and $c$.
\end{thm}
%\simon{The current proof is only for $\sum_{i=1}^{n}\left(\hat{f}(\frac{i}{n})-f(\frac{i}{n})\right)^2$.
%Not exactly 
%$\norm{\hat{f}-f}_2^2$.
%}
The lower bound have two terms.
$\poly\left(L\right)n^{-\frac{2\beta}{2\beta+1}}$ is the classical statistical rate for nonparametric regression.
$\epsilon^2$ represents the contamination dependency.
Notably, the contamination dependency does NOT depend on $L$, Lipschitz constant of function class. 
Or equivalently, it only depends on the noise level.


==> regression_fixed.tex <==
In this section we discuss the local binning median estimator and its theoretical properties.
This estimator combines the idea from robust statistics and nonparametric regression.


We divide the interval $\left[0,1\right]$ into $m$ bins with $j$-th corresponds to the interval $[\frac{num}{den})$ and each bin has $s = \frac{n}{m}$ samples.\footnote{For simplicity of presentation, we assume $m$ and $s$ are both integers. It is straightforward to generalize to the case with $n$ is not a multiple of $s$.}
For a query $x_0$, suppose it is in the $j$-th bin, i.e., $x_0 \in [\left(j-1\right)s,js)$, our estimator is \[
\hat{f}\left(x_0\right) = \median\left\{y_i\right\}_{i=(j-1)s+1}^{js}.
\]




%why we use median
\paragraph{Why Median?} Median is widely used in robust estimation problems for dealing with adversarial noise~\citep{huber2011robust}, heavy tail noise~\citep{brown2008robust}, etc.
There are two fundamentally useful properties about median.
First, median ensure as long as the majority of the samples are good, then the output will not be affected by the small amount of outliers.
Second, median itself has an concentration effect, just like mean.
Our proof heavily relies on these two properties (c.f. Theorem~\ref{thm:fixed_design_median}).

\paragraph{Why Binning}
Binning is used to exploit the smoothness of the function class.
Since the binning estimator only uses observations near the query point, because of the Lipschitz condition of \holder class, this estimator will incur only a small bias.
This is the same idea in kernel smoothing where we often put more weights on points that are near the query point.


Now we analyze the theoretical property of local binning median estimator.
In this section we focus on estimating a function belongs \holder class $\Lambda\left(\beta,L\right)$ with smooth parameter $\beta \le 1$.
The following theorem shows the upper bound of $\ell_2$ risk.
\begin{thm}\label{thm:l2_upper_bound}
	If $m=n^{\frac{1}{1+2\beta}}L^{\frac{2}{2\beta+1}}$, then with high probability\begin{align*}
\norm{\hat{f}-f}_2^2 \le C(L^{\frac{2}{2\beta+1}}n^{-\frac{2\beta}{2\beta+1}}+\epsilon^2).
	\end{align*} 
\end{thm}
Our bound suggests the error comes from two sources.
The first term is the classical statistical rate in non-parametric regression.
The second term represents the contamination dependency.
Notably, this term  but does not depend any property of the function itself, in sharp contrast the naive truncated kernel smoothing estimator we discussed in the last section.

Theorem~\ref{thm:l2_upper_bound} and Theorem~\ref{thm:lower_bound_for_holder} together show that the simple local median binning method is optimal up to absolute constant.
To our knowledge, local binning median is the first computationally efficient method for robust nonparametric regression problem in Huber's $\epsilon$-contamination model with optimal statistical guarantee.

\subsection{Proof of Theorem~\ref{thm:l2_upper_bound}}
In this section, we list the key steps of proving Theorem~\ref{thm:l2_upper_bound}.
The main idea to decouple the error coming from the stochastic noise and from the adversary.

We first focus on the $j$-th bin.
Using some simple deterministic analysis we have the following theorem which shows that we can express the median of each bin as the sum of three terms.
\begin{thm}\label{thm:fixed_design_median}
	Let $z_j = \median\left\{y_i\right\}_{i=(j-1)s}^{js-1}$, then we can write it as\begin{align}
	z_j = f\left(\frac{j}{m}\right) + \eta_j + \triangle_j
	\end{align}
	where \begin{itemize}
		\item $\abs{\triangle_j} \le \max_{\left(j-1\right)s \le i \le js} \abs{f\left(\frac{i}{n}\right) - f\left(\frac{j}{m}\right)}$.
		\item $\eta_j = \median\left\{\xi_i\right\}_{i=(j-1)s}^{js}$.
	\end{itemize} 
\end{thm}
\begin{proof}[Proof of Theorem~\ref{thm:fixed_design_median}]
	Recall we can write $y_i = f\left(\frac{i}{n}\right)+\xi_i$ where $\xi_i \sim \left(1-\epsilon\right)N\left(0,1\right)+\epsilon Q$. 
	Therefore, we have\begin{align*}
	y_i - f\left(\frac{j}{m}\right) = \left(f\left(\frac{i}{n}\right)-f\left(\frac{j}{m}\right)\right)  + \xi_i.
	\end{align*}
	Denote $\eta_j = \median \left\{\xi_i\right\}_{i=(j-1)s}^{js}$.
	Applying Lemma~\ref{thm:median_difference} we have \begin{align*}
	\min_{(j-1)s+1\le i \le js}f\left(\frac{i}{n}\right)\le z_j - \eta_j \le \max_{(j-1)s+1\le i \le js}f\left(\frac{i}{n}\right).
	\end{align*}
	Define $\triangle_j = z_j - \eta_j - f\left(\frac{j}{m}\right)$.
	We can bound it by
	\begin{align*}
	\abs{\triangle_j} \le \max_{\left(j-1\right)s \le i \le js} \abs{f\left(\frac{i}{n}\right) - f\left(\frac{j}{m}\right)}.
	\end{align*}
\end{proof}
The first term is the function value on $\frac{j}{m}$.
If the query point $x_0$ belongs to the $j$-th bin, then $\abs{x_0-\frac{j}{m}}\le \frac{1}{m}$and we have  $\abs{f(x_0)-f(\frac{j}{m})} \le Lm^{-\beta}$ because of the \holder assumption.
This $Lm^{-\beta}$ is ideal bias magnitude in nonparametric regression.
The second term represents the bias due binning.
Note again by the \holder assumption and because the bin length is $\frac{1}{m}$, $\abs{\triangle_j} \le O(Lm^{-\beta})$.
Therefore, it remains to bound the third term, which is main challenge in the analysis.

To analyze $\eta_j$, we use a decoupled analysis for the adversarial noise and stochastic noise.
Suppose in the $j$-th bin, we have $s_j$ observations suffered from the adversarial noise distribution $Q$.
Our key observation is if $s_j \le \frac{s}{4}$, these adversarial points can only incur a small amount of additional bias in the worst case.

\begin{lem}\label{lem:worst_case_adv}
	Let $s,s' \in \mathbb{Z}$, $0 \le s' < \frac{s}{4}$. $\xi_1,\ldots,\xi_{s-s'}$ are fixed numbers and $\xi_{s-s'+1},\ldots,\xi_{s}$ are arbitrary numbers.
	Then \begin{align*}
	\max_{\xi_{s-s'+1},\ldots,\xi_{s}}\median\left\{\xi_i \right\}_{i=1}^s \le \xi_{(\frac{s}{2}:s-s')}\\
	\min_{\xi_{s-s'+1},\ldots,\xi_{s}}\median\left\{\xi_i \right\}_{i=1}^s \ge \xi_{(\frac{s-2s'}{2}:s-s')}
	\end{align*} where $\xi_{(\frac{s}{2}:s-s')}$ and $\xi_{(\frac{s-2s'}{2}:s-s')}$ are the $\frac{s}{2}$-th and the $\frac{s-2s'}{2}$-th largest elements in $\xi_1,\ldots,\xi_{s-s'}$, respectively. 
\end{lem}
\begin{proof}[Proof of Lemma~\ref{lem:worst_case_adv}]
	To maximize the median, we should set $\xi_{s-s'+1},\ldots,\xi_{s} \ge \max\left\{\xi_i\right\}_{i=1}^{s-s'}$ and we get the first inequality.
	The other direction is similar.
\end{proof}

In this lemma, one can think $\xi_1,\ldots,\xi_{s-s'}$ are Gaussian noise and $\xi_{s-s'+1},\ldots,\xi_{s}$ are adversarial noise.
This deterministic lemma shows, if the adversarial points are the minority, then we can control how much they can affect the median estimator.

The requirement of $s_j \le \frac{s}{4}$ is not strongly.
The following lemma shows, this property holds uniformly for all bins with high probability.
\begin{lem}\label{lem:max_adv_in_each_bin}
	Let $s_j$ be number of adversary points in the $j$-th bin, if $s \ge C\log m$ for some absolute constant $C>0$ then with high probability $s_j \le \frac{s}{4}$ for all $j=1,\ldots,m$. 
\end{lem}
\begin{proof}[Proof of Lemma~\ref{lem:max_adv_in_each_bin}]
	Note number of adversarial noise follows a binomial distribution: $s_j \sim \text{ bin}\left(s,\epsilon\right)$.
	Applying Hoeffding inequality, we have \begin{align*}
	\prob\left(s_j \ge s\epsilon + \frac{s}{2}-\epsilon s\right) \le \exp\left(-\frac{2s^2\left(1/2-\epsilon\right)}{s}\right) \le \frac{1}{Cm}.
	\end{align*}
	Using union bound over all bins, we obtain the desired result.
\end{proof}


Therefore, conditioned on $s_j < \frac{s}{4}$  and according to Lemma~\ref{lem:worst_case_adv}, we only need to analyze the $(\frac{s}{2}:s-s_j)$-th and $(\frac{s-2s_j}{2}:s-s_j)$-th quantile of noise from Gaussian distribution.
Now we have successfully decouple the Gaussian noise from the adversarial noise.


The next two lemmas bound the expectation and  variance of quantiles of Gaussian random samples.
They are classical results of sample quantiles~\citep{ruppert2011statistics}.
\begin{lem}[Expectation of Sample Quantile of Gaussian]\label{lem:expectation_of_quantile_gaussian}
	If $s_j \le \frac{s}{4}$, then we have \[\expect{\xi_{(s/2):(s-s_j)}} \le C \frac{s_j}{s} \text{ and } \expect{\xi_{(\frac{s-2s_j}{2}):(s-s_j)}} \ge -C\frac{s_j}{s} \] for some absolute constant $C > 0$.
\end{lem}
\begin{lem}[Variance of Sample Quantile of Gaussian]\label{lem:var_of_quantile_gaussian}
	If $s_j \le \frac{s}{4}$, then we have \[\text{Var}\left(\xi_{(s/2):(s-s_j)}\right) \le \frac{C}{s}\] for some absolute constant $C > 0$.
\end{lem}
Combining Lemma~\ref{lem:worst_case_adv}-Lemma~\ref{lem:var_of_quantile_gaussian}, we have the following bound of $\xi_j$s.
\begin{thm}\label{thm:eta_bound}
If $s \ge c\log m$ for some absolute constant $c >0$ then with high probability, for all $j=1,\ldots,m$ we have \begin{align*}
	\expect{\eta_j^2} \le C\left(\frac{s_j^2}{s^2} + \frac{1}{s}\right)
\end{align*}
for some absolute constant $C>0$ where expectation is over Gaussian noise.
\end{thm}

With these technical results at hand, we are ready to prove the theorem.
We first consider any query point $x$ and suppose it is in the $j$-th bin: $x \in [\frac{j-1}{m},\frac{j}{m})$. 
We can bound the point-wise expected risk \begin{align}
&\expect{\left(\hat{f}\left(x\right)-f\left(x\right)\right)^2} \nonumber \\
=&\expect{
	\left(z_j-f(x)\right)^2
	}\nonumber\\
=&\expect{
	\left(f(\frac{j}{m})+\eta_j+\triangle_j - f(x)\right)^2
	}\nonumber\\
\le & 3\expect{\left(f\left(\frac{j}{m}\right)-f(x)\right)^2 + \eta_j^2+\triangle_j^2} \nonumber\\
\le &3\left(L^2\left(\frac{1}{m}\right)^{2\beta} + C\left(\frac{s_j^2}{s^2} + \frac{1}{s}\right) + L^2\left(\frac{1}{m}\right)^{2\beta} 
\right)\nonumber \\
\triangleq & C_1\left(L^2\left(\frac{1}{m}\right)^{2\beta} +\frac{s_j^2}{s^2} + \frac{1}{s}\right). \label{eqn:pointwise_risk}
\end{align}
The equalities are due to Theorem~\ref{thm:fixed_design_median}.
The first inequality we use $(a+b+c)^2 \le 3(a^2+b^2+c^2)$.
The second inequality we use Theorem~\ref{thm:eta_bound} and the assumption that $f$ belongs to the \holder function class.

Now we can bound the expected $\ell_2$ risk.
\begin{align}
&\expect{\norm{\hat{f}-f}_2^2} \nonumber\\
= & \expect{\int_{0}^{1}\left(\hat{f}(x)-f(x)\right)^2dx} \nonumber \\
 = & \expect{\sum_{j=1}^{m}\int_{\frac{j-1}{m}}^{\frac{j}{m}}(\hat{f}-f(x))^2dx} \nonumber\\
 \le & \frac{1}{m} \sum_{j=1}^{m}C_1\left(L^2\left(\frac{1}{m}\right)^{2\beta} +\frac{s_j^2}{s^2} + \frac{1}{s}\right) \nonumber\\
 = & C_1\left(
L^2\left(\frac{1}{m}\right)^{2\beta} + \frac{\sum_{j=1}^{m}s_j^2}{ms^2}+\frac{1}{s}
\right) \label{eqn:l2_risk}
\end{align} where for the inequality we have used Equation~\eqref{eqn:pointwise_risk}.

Notice that plugging $m\asymp n^{\frac{1}{1+2\beta}}L^{\frac{2}{2\beta+1}}$, we have \begin{align*}
L^2\left(\frac{1}{m}\right)^{2\beta} + \frac{1}{s} \asymp  L^{\frac{2}{2\beta+1}}n^{-\frac{2\beta}{2\beta+1}},
\end{align*} which is the desired statistical rate.

Thus it remains to bound $\frac{s_j^2}{ms^2}$.
Here the power of our decoupled analysis shows up again because this quantity only depends on the number of adversarial points in each bin.
We have the  following lemma.
\begin{lem}\label{lem:square_adv_in_each_bin}
	Let $s_j$ be the number of adversary in the $j$-th bin, then with high probability, \begin{align*}
	\sum_{j=1}^{n}s_j^2 \le C\left(\epsilon s m + s^2\epsilon^2 m\right)
	\end{align*} for some absolute constant $C$.
	\begin{proof}[Proof of Lemma~\ref{lem:square_adv_in_each_bin}]
		Note that $s_j \sim \text{ bin}\left(s,\epsilon\right)$ so we have
		\begin{align*}
		\expect{\sum_{j=1}^{m}s_j^2} = m\left(s^2\epsilon^2+s\epsilon\right).
		\end{align*}
		Now apply Markov's inequality we obtain the desired result.
	\end{proof}
\end{lem}
Lastly, plugging Lemma~\ref{lem:max_adv_in_each_bin} into Equation~\ref{eqn:l2_risk} and using $m\asymp n^{\frac{1}{1+2\beta}}L^{\frac{2}{2\beta+1}}$, we prove Theorem~\ref{thm:l2_upper_bound}.

























==> rel.tex <==
%nonparametric regression applications

%nonparametric regression theory

%robust statistcs classics

%robust nonparametric regression from statistics

%recent regain interest in robust non-parametric
